It's the Best Only When It Fits You Most: Finding Related Models for Serving Based on Dynamic Locality Sensitive Hashing

In recent, deep learning has become the most popular direction in machine learning and artificial intelligence. However, preparation of training data is often a bottleneck in the lifecycle of deploying a deep learning model for production or research. Reusing models for inferencing a dataset can greatly save the human costs required for training data creation. Although there exist a number of model sharing platform such as TensorFlow Hub, PyTorch Hub, DLHub, most of these systems require model uploaders to manually specify the details of each model and model downloaders to screen keyword search results for selecting a model. They are in lack of an automatic model searching tool. This paper proposes an end-to-end process of searching related models for serving based on the similarity of the target dataset and the training datasets of the available models. While there exist many similarity measurements, we study how to efficiently apply these metrics without pair-wise comparison and compare the effectiveness of these metrics. We find that our proposed adaptivity measurement which is based on Jensen-Shannon (JS) divergence, is an effective measurement, and its computation can be significantly accelerated by using the technique of locality sensitive hashing.

==> overlap.tex <==
\section{Overlap Measurement and Metrics}

\subsection{Type-based Metric}
\subsubsection{Type Distance Metric}
The hierarchical type system is a tree structure $T = \{t_i\}$ rooted at node $t_0$, so the distance of any two types is defined as the distance of two tree nodes, as follows. Suppose there are two features/labels $a_i$ and $a_j$. $a_i$ has type $t_i$ and $a_j$ has type $t_j$, which are the two nodes in tree $T$. We denote the distance between $t_i$ and $t_j$ as $d(t_i, t_j)$. If $t_i$ and $t_j$'s lowest common ancestor in $T$ is $t_s$. Then we define that $\forall t_i \in T, d(t_i, t_0) = d(t_0, t_i)= level(t_i)$. In further, we can define that $\forall t_i, t_j \in T, d(t_i, t_j)=(d(t_i, t_0) + d(t_j, t_0)-2\times d(t_0, t_s))/d(t_0, t_s)$. 

\subsubsection{Annotation Similarity Metric}
If both types are annotated, we can further measure the similarity of the annotations.
{\color{red} TODO: How to get the similarity of two types? We can see each annotation as a bag of words, and get the Jaccard similarity. We can train a model to output the similarity. We can ...}

\subsection{Value-based Metrics}
\cite{zhang2020finding, das2012finding}

\subsubsection{Metrics for Numerical Values}
\cite{gonzalez2014three}

\subsubsection{Metrics for Categorical Values}
Boriah and et al.~\cite{boriah2008similarity} lists $14$ similarity measurements for two sets of categorical values.

\subsubsection{Metrics for Array Values}
A number of existing works investigate distance between two clusters~\cite{goldberg2010measuring}

\subsubsection{Metrics for Text Values}
A number of similarity measurements for string values in a github repository~\footnote{ https://github.com/anhaidgroup/py\_stringmatching}. It is also related with entity matching~\cite{li2020deep, zhao2019auto, ebraheem2017deeper, cappuzzo2020creating, fernandez2018seeping}.

\subsubsection{Metrics for Image Values}
KL-divergence, JS-divergence and maximum mean discrepancy?

\subsection{COM: Column-based Overlap Measurement}
TODO: use column-wise comparison to find all matching pairs of columns, then we compute the overall overlap ratio.???

\subsection{TOM: Table-based Overlap Measurement}
TODO: compute the KL-divergence, JS-divergence and maximum mean discrepancy of the overlapped feature space.???

\subsection{GOM: Graph-based Overlap Measurement}
We first introduce how to model a table of raw features and labels into a graph. Every distinct value (an attribute name, a value of an attribute, an annotation if exists, a row key name if exists) is a node, if two different values co-occur in one row or in one column, they are connected by an edge. The weight of the edge is defined as the number of co-occurrences of the two connected nodes. Particularly, if an attribute serves as a label, all distinct label values, label attribute name and annotations are connected to a node "label". 

We can further compress the graph into a super graph, by merging similar nodes (e.g. close numerical values, words with close semantic relationships). For text values, we can transform the two strings into two vectors using a pre-trained word embedding~\cite{}, and then compute the cosine similarity of the two vectors to check whether these two words can be merged into a single node.

Then multiple metrics can be derived to measure the similarity of two super graphs to serve as overlap measurements.



==> problem.tex <==



==> representation.tex <==
\section{Domain Representations}
We advocate for using raw features and labels to represent the domain of a deep learning problem. Each feature or label is associated hierarchical types and will be represented differently depending on its types.

\subsection{Feature Types}
Two raw features can overlap at different granularity. For example, a set of movie names and a set of music names can be regarded as similar, because the values of both features are texts. But these two features are actually describing two different domains, so they are not exactly the same.

To represent such different levels of matching semantics, we associate a hierarchical relationship with each feature/label: the highest-level type to describe the property associated with the feature, such as numeric, datetime, boolean, categorical (enumerator), text, image, binary, and so on; and then a lower-level type to describe the domains associated with the feature, for example, a text-based feature may describe locations, people names, organization names, publication titles and so on; in further, a feature which is classified as publication titles can be further divided into movie titles, music titles, article titles, book titles and so on. Similarly, a numerical feature can be divided into multiple levels based on different ranges, different shapes of distribution, different levels of precision, etc..

{\color{red} TODO: How to get hierarchical types? Can we create a hierarchical classifier leveraging an open-source Named Entity Recognition (NER) model or Bing knowledge graph?}

\subsection{Feature/Label Values}
All values associated with a feature/label in the training dataset formulates a value set for the feature/label. Depending on the highest-level type of the feature/label, we can represent its value set differently.
\subsubsection{Numerical Values}


\subsubsection{Categorical Values}
{\color{red}{Optional for the first version?}}

\subsubsection{Array Values}

\subsubsection{Texts}

\subsubsection{Images}

\subsubsection{Binaries}
{\color{red}{Optional for the first version?}}

\subsection{Feature/Label Name or Annotations}
Sometimes, when raw features and the label are stored in a CSV file or other structured formats, we may find names (e.g. in the header of a CSV file) or annotations that describe a feature or label.

==> system.tex <==
\section{System Architecture and Implementation}

